A Blockchain-based Flight Data Recorder for Cloud Accountability

Many companies rely on Cloud infrastructures for their computation, communication and data storage requirements. While Cloud services provide some benefits, e.g., replacing high upfront costs for an IT infrastructure with a pay-as-you-go model, they also introduce serious concerns that are notoriously difficult to address. In essence, Cloud customers are storing data and running computations on infrastructures that they can not control directly. Therefore, when problems arise -- violations of Service Level Agreements, data corruption, data leakage, security breaches -- both customers and Cloud providers face the challenge of agreeing on which party is to be held responsible. In this paper, we review the challenges and requirements for enforcing accountability in Cloud infrastructures, and argue that smart contracts and blockchain technologies might provide a key contribution towards accountable Clouds.

==> Makefile <==
DOC=cloud-accountability
CR=cloud-accountability
CHAPTERS=$(wildcard *.tex)
MAKEDEPEND=(echo -n "FIGS=" && cat $(DOC).tex $(CHAPTERS) | perl -ne 'if (m/^[^%]*\\includegraphics.*\{([^\}]+)\}/) { print $$1 . ".eps " }' && echo ) > $(DOC).dep

-include $(DOC).dep

.PHONY: update_figs clean

ALL: pdf

ps: $(CR).ps

pdf: $(CR).pdf

$(DOC).dep: $(DOC).tex $(CHAPTERS)
	@$(MAKEDEPEND)

$(CR).ps: $(DOC).dvi
#	dvips -t letter $< -o $(CR).ps

$(CR).pdf: $(CR).ps
#	ps2pdf -dPDFSETTINGS=/prepress -dSubsetFonts=true -dEmbedAllFonts=true $< tmp.pdf && qpdf --linearize tmp.pdf $@ && rm -f tmp.pdf

$(DOC).dvi: $(DOC).tex $(DOC).bib $(CHAPTERS)
	pdflatex $(DOC) && bibtex $(DOC) && pdflatex $(DOC) && pdflatex $(DOC)

clean:
	\rm -f *~ *.aux *.bbl *.blg *.log $(DOC).dvi $(DOC).ps $(DOC).pdf $(CR).ps $(CR).pdf $(DOC).dep
#	$(MAKE) -C graphs clean


==> sec-challenges.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Requirements}\label{sec:requirements}

Accountability is fundamental to developing trust in services.  This
Project takes inspiration from the civil aviation industry and
proposes a novel approach of creating a ``flight recorder'' for the
cloud that records service interaction events at sufficiently fine
granularity in to enable investigations of accidents or incidents.
Development of CEDAR requires answering two questions: what to record
and how to record. CEDAR objectives 1 and 2 essentially address 'what'
and objective 3 addresses 'how'. In this project we recognize that the
issues raised can not be addressed only from a technical point of
view, but it is also necessary to consider all legal implications. For
this reason, the project requires expertise of both computer
scientists and legal scholars. Thus, all technical solutions will be
evaluated in light view of current European law, in order to ensure
that CEDAR is capable of producing evidences that can stand up in
court.  We consider 'how' first.  CEDAR must provide a
tamper‐resistant, trustworthy log, which can be considered, in
accordance with present legislation, as a reliable document with legal
value.  Logging in CEDAR should have the following characteristics:
logging must guarantee fairness and non‐repudiation, ensuring that
well‐behaved parties are not disadvantaged by the misbehaviour of
others and that no party can subsequently deny their participation.
it should enable tracing back the causes of an 'incident' (behaviour
that is not contract compliant, that is, deviation from
expected/legitimate behaviour) after it has occurred; its presence
must not limit the functioning and the types of services offered by
the cloud itself; logging itself should be constructed using cloud
computing services.  It is an open question at the moment whether such
logging is feasible.  For this reason, CEDAR aims to create the
scientific foundations of secure logging in a potentially hostile
environment. It will explore multilateral security mechanisms that
take account of the (possibly conflicting) interests of all parties
(e.g. preferring mutual authentication to unilateral authentication of
users by a service).  Cloud providers and cloud users require
protection with respect to each other’s actions, with provider
assurances rooted in an independent source of trust.  For example,
there should be user‐verifiable assurance that the applications and
services they deploy in the cloud are secure against compromise by
cloud provider system administrators.  We consider 'what' next. Cloud
Computing creates new relationships between an organization and third
party cloud service providers, posing new challenges in understanding
how laws apply in a wide variety of information management scenarios.
A contracted cloud provider might itself use subcontractors, over whom
the cloud user has no control.  The general scenario is that cloud
services could be arbitrarily complex, dynamically composed from
varieties of services (ranging from computational, storage, network to
application level) provided by globally distributed service
providers. Service providers will offer their services to consumers
with specific quality of service (QoS) attributes, such as
reliability, security, under specific terms and conditions; there will
be financial penalties if the requirements are not met.  A service
consumer composing an application--a composite service--will also be
expected to offer QoS guarantees, covering robustness and security,
with financial accountability to their consumers under specific terms
and conditions. This process can be arbitrarily nested.  Most of the
existing research on SLA management focuses on computational and
algorithmic aspects of QoS monitoring and provision. Specifically,
considerable effort has been spent so far in developing proactive or
reactive algorithms for allocating the appropriate number and kind of
resources needed to meet a set of given QoS requirements;
unfortunately, despite every effort SLA violations do happen in
practice, and it is necessary to deal with them. So far, SLA
violations must be handled entirely on the basis of ``out of band''
negotiations between service providers and service consumers since the
systems being monitored are currently unable to provide legal
evidences of malfunctions (or lack of).  This may result in long and
costly litigations, which are harmful to both the service provider and
its customers. The lack of a well-defined framework for identifying
violations and assigning responsibilities is a limiting factor towards
the adoption of clouds for critical applications (real-time data
processing, health care, financial applications and so on).  With
CEDAR, we intend to change the above situation. We realise that it is
inherently difficult to identify responsibilities when the business
agreements do not respect expectations or violate contractual
obligations. Clearly, all constraints and violations that need to be
monitored must be identified.  A bewilderingly wide spectrum of
possibilities exists; examples include constraints on availability and
response time requirements, constraints on the geographical locations
of physical resources of the cloud where data can be stored and
processed.  This latter issue is a extremely delicate issue, as it may
also involve ``friendly'' countries. For instance, the Canadian
government has a policy of not allowing public sector IT projects to
use US‐based hosting services because of concerns over data
protection.  CEDAR aims to create the scientific foundations of
managing business relationships electronically. It will provide ways
of formulating machine interpretable sets of rules -- electronic
contracts -- from service contracts that are typically written in
legal English. Such electronic contracts will contain two kind of
contractual clauses: terms and conditions and SLAs.  Terms and
conditions are concerned with rights, obligations and prohibitions to
perform a particular action (eg., delete a file, make a payment,
etc.); whereas SLAs are concerned with right, obligations and
prohibitions to maintain a given service in a particular state
(eg. running Mon‐Fri with a response time less than one second).

Electronic contracts will form the basis of systematically determining
monitoring requirements for detecting rule violations by recording
service interactions at a granularity that is sufficient for checking
that they comply with the rights (permissions), obligations and
prohibitions stipulated in contract clauses and tracing causes of
violations. Recording service interactions must resolve the tension
between recording at micro-level (recording events at too fine-grained
level could seriously degrade the perform ace of the offered service)
and macro-level (some important information is missed).

